AXES: Approximation Manager for Emerging Memory Architectures

Memory approximation techniques are commonly limited in scope, targeting individual levels of the memory hierarchy. Existing approximation techniques for a full memory hierarchy determine optimal configurations at design-time provided a goal and application. Such policies are rigid: they cannot adapt to unknown workloads and must be redesigned for different memory configurations and technologies. We propose AXES: the first self-optimizing runtime manager for coordinating configurable approximation knobs across all levels of the memory hierarchy. AXES continuously updates and optimizes its approximation management policy throughout runtime for diverse workloads. AXES optimizes the approximate memory configuration to minimize power consumption without compromising the quality threshold specified by application developers. AXES can (1) learn a policy at runtime to manage variable application quality of service (QoS) constraints, (2) automatically optimize for a target metric within those constraints, and (3) coordinate runtime decisions for interdependent knobs and subsystems. We demonstrate AXES' ability to efficiently provide functions 1-3 on a RISC-V Linux platform with approximate memory segments in the on-chip cache and main memory. We demonstrate AXES' ability to save up to 37% energy in the memory subsystem without any design-time overhead. We show AXES' ability to reduce QoS violations by 75% with $<5\%$ additional energy.

==> figs/experiments/blackscholes/exp_blk_c.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
height=3cm,
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xlabel={Frame},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel={\(\displaystyle V_{DD}\)},
ymajorgrids,
ymin=1, ymax=4,
ytick style={color=black},
ytick={1,2,3,4},
yticklabels={0.7V,0.8V,0.9V,1.0V}
]
\addplot [line width=1pt, color0]
table {%
1 3
2 3
3 3
4 2
5 3
6 2
7 3
8 3
9 3
10 3
11 3
12 3
13 3
14 3
15 3
16 3
17 3
18 3
19 3
20 3
21 3
22 3
23 3
24 3
25 3
26 3
27 3
28 3
29 2
30 3
31 2
32 1
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 1
62 2
63 1
64 1
65 1
66 1
67 1
68 1
69 1
70 1
71 1
72 1
73 1
74 1
75 1
76 1
77 1
78 1
79 1
80 1
81 1
82 1
83 1
84 1
85 1
86 1
87 1
88 1
89 2
90 2
91 2
92 2
93 2
94 2
95 2
96 2
97 2
98 2
99 2
};
\addlegendentry{L1D}
\addplot [line width=1pt, color1]
table {%
1 2
2 3
3 3
4 2
5 1
6 1
7 1
8 1
9 1
10 1
11 1
12 1
13 1
14 1
15 1
16 1
17 1
18 1
19 1
20 1
21 1
22 1
23 1
24 1
25 1
26 1
27 1
28 1
29 1
30 1
31 1
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 1
66 1
67 2
68 2
69 1
70 1
71 1
72 1
73 1
74 2
75 2
76 2
77 2
78 2
79 2
80 2
81 2
82 2
83 2
84 2
85 2
86 2
87 2
88 2
89 2
90 2
91 2
92 2
93 2
94 2
95 2
96 2
97 2
98 2
99 2
};
\addlegendentry{L2}
\end{axis}

\end{tikzpicture}


==> figs/experiments/blackscholes/exp_blk_d.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
height=3cm,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xlabel={Frame},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel={Refresh cycle},
ymajorgrids,
ymin=1, ymax=4,
ytick style={color=black},
ytick={1,2,3,4},
yticklabels={20s,5s,1s,0.1s}
]
\addplot [line width=1pt, color0]
table {%
1 2
2 2
3 3
4 3
5 3
6 3
7 2
8 2
9 2
10 2
11 2
12 2
13 2
14 2
15 2
16 2
17 2
18 2
19 2
20 2
21 2
22 2
23 2
24 2
25 2
26 2
27 2
28 2
29 3
30 2
31 1
32 0
33 1
34 2
35 2
36 2
37 2
38 2
39 2
40 2
41 2
42 2
43 2
44 2
45 2
46 2
47 2
48 2
49 2
50 2
51 2
52 2
53 2
54 2
55 2
56 2
57 2
58 2
59 2
60 2
61 1
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
80 0
81 0
82 0
83 0
84 0
85 0
86 0
87 0
88 0
89 0
90 0
91 0
92 0
93 0
94 0
95 0
96 0
97 0
98 0
99 0
};
\addlegendentry{DRAM}
\end{axis}

\end{tikzpicture}


==> figs/experiments/blackscholes/exp_blk_qos.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 5}]
\nextgroupplot[
height=3cm,
legend cell align={left},
legend columns=2,
legend style={fill opacity=1, draw opacity=1, text opacity=1, at={(0.5,1.2)}, anchor=north, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel style={align=center}, ylabel={Avg. Rel.\\Error},
ymajorgrids,
ymin=0, ymax=45,
ytick style={color=black},
ytick={0,10,20,30,40}
]
\addplot [line width=1pt, black, dashed]
table {%
1 5
2 5
3 5
4 5
5 5
6 5
7 5
8 5
9 5
10 5
11 5
12 5
13 5
14 5
15 5
16 5
17 5
18 5
19 5
20 5
21 5
22 5
23 5
24 5
25 5
26 5
27 5
28 5
29 5
30 30
31 30
32 30
33 30
34 30
35 30
36 30
37 30
38 30
39 30
40 30
41 30
42 30
43 30
44 30
45 30
46 30
47 30
48 30
49 30
50 30
51 30
52 30
53 30
54 30
55 30
56 30
57 30
58 30
59 30
60 12
61 12
62 12
63 12
64 12
65 12
66 12
67 12
68 12
69 12
70 12
71 12
72 12
73 12
74 12
75 12
76 12
77 12
78 12
79 12
80 12
81 12
82 12
83 12
84 12
85 12
86 12
87 12
88 12
89 12
90 12
91 12
92 12
93 12
94 12
95 12
96 12
97 12
98 12
99 12
};
\addlegendentry{QoS Constraint}
\addplot [line width=1pt, color0]
table {%
1 2.392728
2 2.381114
3 2.377069
4 2.409615
5 2.450321
6 2.377058
7 2.474078
8 2.49833
9 2.377206
10 2.449828
11 2.681162
12 2.904194
13 2.750757
14 2.685881
15 2.70964
16 2.624537
17 2.666653
18 2.598519
19 2.61968
20 2.634361
21 2.574903
22 2.593171
23 2.794069
24 2.930253
25 2.670474
26 2.719951
27 2.841158
28 2.841053
29 2.624162
30 2.68586
31 9.730583
32 8.807265
33 8.542678
34 9.469681
35 27.688057
36 27.380358
37 28.186071
38 27.432465
39 27.992616
40 26.796509
41 27.837089
42 26.985281
43 27.391266
44 27.720905
45 27.071396
46 27.631064
47 28.322625
48 27.833221
49 27.946701
50 27.989751
51 27.557181
52 26.793273
53 27.705249
54 29.85129
55 12.710313
56 27.471289
57 28.089746
58 28.948309
59 27.925755
60 26.690438
61 24.099658
62 3.685525
63 9.213044
64 9.460122
65 9.171839
66 9.471212
67 9.288253
68 8.825161
69 8.989663
70 9.81984
71 9.73862
72 8.935846
73 10.081864
74 10.755716
75 9.225509
76 9.008018
77 8.610445
78 9.156304
79 8.992528
80 8.695229
81 8.924771
82 9.4938
83 12.35329
84 12.655116
85 12.816662
86 6.207539
87 5.035616
88 5.100364
89 5.272721
90 5.16946
91 5.09463
92 5.211537
93 3.831082
94 6.352766
95 6.254967
96 9.234445
97 9.574241
98 9.209946
99 8.943507
};
\addlegendentry{\seams{} 1}
\addplot [line width=0.5pt, blue, mark=|, mark size=2, mark options={solid}, only marks, forget plot]
table {%
1 2.392728
2 2.381114
3 2.377069
4 2.409615
5 2.450321
6 2.377058
7 2.474078
8 2.49833
9 2.377206
10 2.449828
11 2.681162
12 2.904194
13 2.750757
14 2.685881
15 2.70964
16 2.624537
17 2.666653
18 2.598519
19 2.61968
20 2.634361
21 2.574903
22 2.593171
23 2.794069
24 2.930253
25 2.670474
26 2.719951
27 2.841158
28 2.841053
29 2.624162
30 2.68586
31 9.730583
32 8.807265
33 8.542678
34 9.469681
35 27.688057
36 27.380358
37 28.186071
38 27.432465
39 27.992616
40 26.796509
41 27.837089
42 26.985281
43 27.391266
44 27.720905
45 27.071396
46 27.631064
47 28.322625
48 27.833221
49 27.946701
50 27.989751
51 27.557181
52 26.793273
53 27.705249
54 29.85129
55 12.710313
56 27.471289
57 28.089746
58 28.948309
59 27.925755
60 26.690438
61 24.099658
62 3.685525
63 9.213044
64 9.460122
65 9.171839
66 9.471212
67 9.288253
68 8.825161
69 8.989663
70 9.81984
71 9.73862
72 8.935846
73 10.081864
74 10.755716
75 9.225509
76 9.008018
77 8.610445
78 9.156304
79 8.992528
80 8.695229
81 8.924771
82 9.4938
83 12.35329
84 12.655116
85 12.816662
86 6.207539
87 5.035616
88 5.100364
89 5.272721
90 5.16946
91 5.09463
92 5.211537
93 3.831082
94 6.352766
95 6.254967
96 9.234445
97 9.574241
98 9.209946
99 8.943507
};

\nextgroupplot[
height=3cm,
legend cell align={left},
legend columns=2,
legend style={fill opacity=1, draw opacity=1, text opacity=1, at={(0.5,1.2)}, anchor=north, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel style={align=center}, ylabel={Avg. Rel.\\Error},
ymajorgrids,
ymin=0, ymax=45,
ytick style={color=black},
ytick={0,10,20,30,40}
]
\addplot [line width=1pt, black, dashed]
table {%
1 5
2 5
3 5
4 5
5 5
6 5
7 5
8 5
9 5
10 5
11 5
12 5
13 5
14 5
15 5
16 5
17 5
18 5
19 5
20 5
21 5
22 5
23 5
24 5
25 5
26 5
27 5
28 5
29 5
30 30
31 30
32 30
33 30
34 30
35 30
36 30
37 30
38 30
39 30
40 30
41 30
42 30
43 30
44 30
45 30
46 30
47 30
48 30
49 30
50 30
51 30
52 30
53 30
54 30
55 30
56 30
57 30
58 30
59 30
60 12
61 12
62 12
63 12
64 12
65 12
66 12
67 12
68 12
69 12
70 12
71 12
72 12
73 12
74 12
75 12
76 12
77 12
78 12
79 12
80 12
81 12
82 12
83 12
84 12
85 12
86 12
87 12
88 12
89 12
90 12
91 12
92 12
93 12
94 12
95 12
96 12
97 12
98 12
99 12
};
\addlegendentry{QoS Constraint}
\addplot [line width=1pt, color0]
table {%
1 2.392728
2 2.733618
3 5.082575
4 5.08719
5 5.111408
6 5.40853
7 5.286533
8 5.166604
9 5.275383
10 5.015127
11 5.23245
12 3.215826
13 3.50108
14 3.415969
15 3.320052
16 3.552444
17 3.552096
18 3.374829
19 3.180041
20 3.392868
21 3.331922
22 3.535014
23 3.41204
24 3.408278
25 3.331918
26 3.066427
27 3.413074
28 3.5216
29 3.478553
30 3.571065
31 5.682811
32 5.182374
33 6.360785
34 28.038229
35 27.797985
36 28.307094
37 27.836554
38 26.712408
39 28.003462
40 26.27498
41 27.837089
42 26.985281
43 27.391266
44 27.720905
45 27.071396
46 27.631064
47 28.322625
48 3.910652
49 3.710869
50 22.498318
51 23.13447
52 26.793273
53 27.705249
54 28.075455
55 27.526746
56 27.471289
57 28.089746
58 28.948309
59 27.925755
60 26.690438
61 9.794399
62 9.816718
63 10.126163
64 10.122996
65 9.700376
66 9.609838
67 10.626555
68 9.606159
69 9.87491
70 9.845915
71 9.5104
72 9.517833
73 9.818647
74 9.602955
75 9.225509
76 9.008018
77 8.610445
78 9.156304
79 9.129047
80 8.695229
81 8.924771
82 9.4938
83 9.222419
84 9.124477
85 9.611974
86 9.334524
87 10.209145
88 9.321527
89 10.108621
90 6.129325
91 6.115672
92 5.211537
93 5.017524
94 5.276655
95 5.334307
96 4.93397
97 5.179316
98 5.121304
99 5.310211
};
\addlegendentry{\seams{} 2}
\addplot [line width=0.5pt, blue, mark=|, mark size=2, mark options={solid}, only marks, forget plot]
table {%
1 2.392728
2 2.733618
3 5.082575
4 5.08719
5 5.111408
6 5.40853
8 5.166604
10 5.015127
12 3.215826
14 3.415969
16 3.552444
18 3.374829
20 3.392868
22 3.535014
24 3.408278
26 3.066427
28 3.5216
30 3.571065
31 5.682811
32 5.182374
33 6.360785
34 28.038229
36 28.307094
38 26.712408
40 26.27498
42 26.985281
44 27.720905
46 27.631064
48 3.910652
50 22.498318
52 26.793273
54 28.075455
56 27.471289
58 28.948309
60 26.690438
61 9.794399
62 9.816718
63 10.126163
64 10.122996
66 9.609838
68 9.606159
70 9.845915
72 9.517833
74 9.602955
76 9.008018
78 9.156304
80 8.695229
82 9.4938
84 9.124477
86 9.334524
88 9.321527
90 6.129325
92 5.211537
94 5.276655
96 4.93397
98 5.121304
};

\nextgroupplot[
height=3cm,
legend cell align={left},
legend columns=2,
legend style={fill opacity=1, draw opacity=1, text opacity=1, at={(0.5,1.2)}, anchor=north, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel style={align=center}, ylabel={Avg. Rel.\\Error},
ymajorgrids,
ymin=0, ymax=45,
ytick style={color=black},
ytick={0,10,20,30,40}
]
\addplot [line width=1pt, black, dashed]
table {%
1 5
2 5
3 5
4 5
5 5
6 5
7 5
8 5
9 5
10 5
11 5
12 5
13 5
14 5
15 5
16 5
17 5
18 5
19 5
20 5
21 5
22 5
23 5
24 5
25 5
26 5
27 5
28 5
29 5
30 30
31 30
32 30
33 30
34 30
35 30
36 30
37 30
38 30
39 30
40 30
41 30
42 30
43 30
44 30
45 30
46 30
47 30
48 30
49 30
50 30
51 30
52 30
53 30
54 30
55 30
56 30
57 30
58 30
59 30
60 12
61 12
62 12
63 12
64 12
65 12
66 12
67 12
68 12
69 12
70 12
71 12
72 12
73 12
74 12
75 12
76 12
77 12
78 12
79 12
80 12
81 12
82 12
83 12
84 12
85 12
86 12
87 12
88 12
89 12
90 12
91 12
92 12
93 12
94 12
95 12
96 12
97 12
98 12
99 12
};
\addlegendentry{QoS Constraint}
\addplot [line width=1pt, color0]
table {%
1 2.392728
2 2.733618
3 11.486602
4 9.300339
5 9.454109
6 9.591792
7 9.05337
8 8.77055
9 9.701514
10 2.825952
11 2.93282
12 2.916585
13 2.840021
14 2.799703
15 2.844986
16 2.876505
17 2.850136
18 2.92904
19 2.696628
20 2.796095
21 2.809522
22 2.815703
23 2.923998
24 2.998914
25 2.718551
26 2.889768
27 2.837355
28 2.704939
29 2.87159
30 2.896257
31 9.97732
32 29.0772
33 22.38274
34 28.038229
35 27.797985
36 28.307094
37 27.836554
38 26.712408
39 28.003462
40 26.27498
41 27.837089
42 26.985281
43 27.391266
44 27.720905
45 27.071396
46 27.631064
47 28.322625
48 27.833221
49 27.946701
50 27.989751
51 27.557181
52 26.793273
53 27.705249
54 28.075455
55 27.526746
56 27.471289
57 28.089746
58 28.948309
59 27.925755
60 26.690438
61 9.794399
62 9.816718
63 10.126163
64 10.122996
65 28.375501
66 27.65301
67 28.17861
68 27.006479
69 27.513054
70 10.090624
71 10.683711
72 9.365892
73 10.081864
74 10.755716
75 9.657731
76 10.164909
77 10.809741
78 9.876124
79 10.430352
80 9.863653
81 9.709227
82 9.86531
83 10.168515
84 10.185337
85 9.792011
86 9.135744
87 9.813006
88 10.360343
89 9.817017
90 9.494588
91 9.76119
92 8.840022
93 9.143154
94 9.416831
95 9.393825
96 8.988625
97 9.438452
98 9.652701
99 9.088224
};
\addlegendentry{\seams{} 5}
\addplot [line width=0.5pt, blue, mark=|, mark size=2, mark options={solid}, only marks, forget plot]
table {%
1 2.392728
2 2.733618
3 11.486602
4 9.300339
5 9.454109
10 2.825952
15 2.844986
20 2.796095
25 2.718551
30 2.896257
31 9.97732
32 29.0772
33 22.38274
34 28.038229
35 27.797985
40 26.27498
45 27.071396
50 27.989751
55 27.526746
60 26.690438
61 9.794399
62 9.816718
63 10.126163
64 10.122996
65 28.375501
70 10.090624
75 9.657731
80 9.863653
85 9.792011
90 9.494588
95 9.393825
};

\nextgroupplot[
height=3cm,
legend cell align={left},
legend columns=2,
legend style={fill opacity=1, draw opacity=1, text opacity=1, at={(0.5,1.2)}, anchor=north, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel style={align=center}, ylabel={Avg. Rel.\\Error},
ymajorgrids,
ymin=0, ymax=45,
ytick style={color=black},
ytick={0,10,20,30,40}
]
\addplot [line width=1pt, black, dashed]
table {%
1 5
2 5
3 5
4 5
5 5
6 5
7 5
8 5
9 5
10 5
11 5
12 5
13 5
14 5
15 5
16 5
17 5
18 5
19 5
20 5
21 5
22 5
23 5
24 5
25 5
26 5
27 5
28 5
29 5
30 30
31 30
32 30
33 30
34 30
35 30
36 30
37 30
38 30
39 30
40 30
41 30
42 30
43 30
44 30
45 30
46 30
47 30
48 30
49 30
50 30
51 30
52 30
53 30
54 30
55 30
56 30
57 30
58 30
59 30
60 12
61 12
62 12
63 12
64 12
65 12
66 12
67 12
68 12
69 12
70 12
71 12
72 12
73 12
74 12
75 12
76 12
77 12
78 12
79 12
80 12
81 12
82 12
83 12
84 12
85 12
86 12
87 12
88 12
89 12
90 12
91 12
92 12
93 12
94 12
95 12
96 12
97 12
98 12
99 12
};
\addlegendentry{QoS Constraint}
\addplot [line width=1pt, color0]
table {%
1 2.392728
2 2.733618
3 11.486602
4 9.300339
5 3.419391
6 3.803021
7 3.490755
8 3.727568
9 3.66814
10 3.409294
11 3.702597
12 4.002552
13 3.5375
14 3.460033
15 3.465934
16 3.469795
17 3.682448
18 3.427912
19 3.774992
20 3.664995
21 3.700237
22 3.179923
23 3.796146
24 3.716995
25 3.763097
26 3.369316
27 3.471514
28 3.704051
29 3.401443
30 3.603561
31 27.518138
32 28.070588
33 27.82428
34 28.038229
35 27.797985
36 28.307094
37 27.836554
38 26.712408
39 28.003462
40 26.27498
41 27.837089
42 26.985281
43 27.391266
44 27.720905
45 27.071396
46 27.631064
47 28.322625
48 27.833221
49 27.946701
50 27.989751
51 27.557181
52 26.793273
53 27.705249
54 28.075455
55 27.526746
56 27.471289
57 28.089746
58 28.948309
59 27.925755
60 3.7998
61 9.267306
62 6.424647
63 4.929297
64 5.197565
65 4.988772
66 5.262863
67 5.006226
68 5.247262
69 5.041683
70 5.117714
71 5.525036
72 5.274646
73 5.17805
74 5.31678
75 5.259862
76 5.113098
77 5.226029
78 5.037605
79 5.251458
80 5.50101
81 5.333805
82 4.945678
83 5.168202
84 5.170564
85 5.304162
86 5.173666
87 5.035616
88 5.100364
89 5.272721
90 5.16946
91 5.09463
92 5.211537
93 5.017524
94 5.276655
95 5.334307
96 4.93397
97 5.179316
98 5.121304
99 5.310211
};
\addlegendentry{\seams{} 10}
\addplot [line width=0.5pt, blue, mark=|, mark size=2, mark options={solid}, only marks, forget plot]
table {%
1 2.392728
2 2.733618
3 11.486602
4 9.300339
5 3.419391
10 3.409294
20 3.664995
30 3.603561
31 27.518138
32 28.070588
33 27.82428
34 28.038229
40 26.27498
50 27.989751
60 3.7998
61 9.267306
62 6.424647
63 4.929297
64 5.197565
70 5.117714
80 5.50101
90 5.16946
};

\nextgroupplot[
height=3cm,
legend cell align={left},
legend columns=2,
legend style={fill opacity=1, draw opacity=1, text opacity=1, at={(0.5,1.2)}, anchor=north, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel style={align=center}, ylabel={Avg. Rel.\\Error},
ymajorgrids,
ymin=0, ymax=45,
ytick style={color=black},
ytick={0,10,20,30,40}
]
\addplot [line width=1pt, black, dashed]
table {%
1 5
2 5
3 5
4 5
5 5
6 5
7 5
8 5
9 5
10 5
11 5
12 5
13 5
14 5
15 5
16 5
17 5
18 5
19 5
20 5
21 5
22 5
23 5
24 5
25 5
26 5
27 5
28 5
29 5
30 30
31 30
32 30
33 30
34 30
35 30
36 30
37 30
38 30
39 30
40 30
41 30
42 30
43 30
44 30
45 30
46 30
47 30
48 30
49 30
50 30
51 30
52 30
53 30
54 30
55 30
56 30
57 30
58 30
59 30
60 12
61 12
62 12
63 12
64 12
65 12
66 12
67 12
68 12
69 12
70 12
71 12
72 12
73 12
74 12
75 12
76 12
77 12
78 12
79 12
80 12
81 12
82 12
83 12
84 12
85 12
86 12
87 12
88 12
89 12
90 12
91 12
92 12
93 12
94 12
95 12
96 12
97 12
98 12
99 12
};
\addlegendentry{QoS Constraint}
\addplot [line width=1pt, color0]
table {%
1 2.392728
2 2.733618
3 11.486602
4 9.300339
5 3.419391
6 3.803021
7 3.490755
8 3.727568
9 3.66814
10 3.409294
11 3.702597
12 4.002552
13 3.5375
14 3.460033
15 3.465934
16 3.469795
17 3.682448
18 3.427912
19 3.774992
20 3.664995
21 3.700237
22 3.179923
23 3.796146
24 3.716995
25 3.763097
26 3.369316
27 3.471514
28 3.704051
29 3.401443
30 3.603561
31 27.518138
32 28.070588
33 27.82428
34 28.038229
35 27.797985
36 28.307094
37 27.836554
38 26.712408
39 28.003462
40 26.27498
41 27.837089
42 26.985281
43 27.391266
44 27.720905
45 27.071396
46 27.631064
47 28.322625
48 27.833221
49 27.946701
50 27.989751
51 27.557181
52 26.793273
53 27.705249
54 28.075455
55 27.526746
56 27.471289
57 28.089746
58 28.948309
59 27.925755
60 26.690438
61 9.794399
62 9.816718
63 9.157276
64 9.888298
65 9.95058
66 9.353797
67 9.469209
68 9.606159
69 9.87491
70 9.845915
71 9.5104
72 9.517833
73 9.818647
74 9.602955
75 9.225509
76 9.008018
77 8.610445
78 9.197398
79 8.996969
80 9.618279
81 9.290258
82 9.113731
83 9.143666
84 9.337679
85 8.866523
86 9.143297
87 8.900086
88 9.140816
89 9.263039
90 9.494588
91 9.76119
92 8.840022
93 9.143154
94 9.416831
95 9.393825
96 8.988625
97 9.438452
98 9.652701
99 9.088224
};
\addlegendentry{\seams{} 20}
\addplot [line width=0.5pt, blue, mark=|, mark size=2, mark options={solid}, only marks, forget plot]
table {%
1 2.392728
2 2.733618
3 11.486602
4 9.300339
5 3.419391
20 3.664995
30 3.603561
31 27.518138
32 28.070588
33 27.82428
34 28.038229
40 26.27498
60 26.690438
61 9.794399
62 9.816718
63 9.157276
64 9.888298
80 9.618279
};
\end{groupplot}
\end{tikzpicture}


==> figs/experiments/kmeans/exp_kmeans_c.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
height=3cm,
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xlabel={Frame},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel={\(\displaystyle V_{DD}\)},
ymajorgrids,
ymin=1, ymax=4,
ytick style={color=black},
ytick={1,2,3,4},
yticklabels={0.7V,0.8V,0.9V,1.0V}
]
\addplot [line width=1pt, color0]
table {%
1 3
2 3
3 3
4 3
5 3
6 3
7 3
8 3
9 3
10 3
11 3
12 3
13 3
14 3
15 3
16 3
17 3
18 3
19 3
20 3
21 3
22 3
23 3
24 3
25 3
26 3
27 3
28 3
29 3
30 3
31 3
32 3
33 2
34 2
35 1
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 1
62 1
63 1
64 1
65 1
66 1
67 1
68 1
69 1
70 1
71 1
72 1
73 1
74 1
75 1
76 1
77 1
78 1
79 1
80 1
81 1
82 1
83 1
84 1
85 1
86 1
87 1
88 1
89 1
90 1
91 1
92 1
93 1
94 1
95 1
96 1
97 1
98 1
99 1
};
\addlegendentry{L1D}
\addplot [line width=1pt, color1]
table {%
1 2
2 2
3 2
4 2
5 2
6 2
7 2
8 2
9 2
10 2
11 2
12 2
13 2
14 2
15 2
16 2
17 2
18 2
19 2
20 2
21 2
22 2
23 2
24 2
25 2
26 2
27 2
28 2
29 2
30 2
31 2
32 1
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
80 0
81 0
82 0
83 0
84 0
85 0
86 0
87 0
88 0
89 0
90 0
91 0
92 0
93 0
94 0
95 0
96 0
97 0
98 0
99 0
};
\addlegendentry{L2}
\end{axis}

\end{tikzpicture}


==> figs/experiments/kmeans/exp_kmeans_d.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
height=3cm,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.0196078431373!black},
xlabel={Frame},
xmin=-3.9, xmax=103.9,
xtick style={color=black},
xtick={-20,0,20,40,60,80,100,120},
y grid style={white!69.0196078431373!black},
ylabel={Refresh cycle},
ymajorgrids,
ymin=1, ymax=4,
ytick style={color=black},
ytick={1,2,3,4},
yticklabels={20s,5s,1s,0.1s}
]
\addplot [line width=1pt, color0]
table {%
1 3
2 3
3 3
4 3
5 3
6 3
7 3
8 3
9 3
10 3
11 3
12 3
13 3
14 3
15 3
16 3
17 3
18 3
19 3
20 3
21 3
22 3
23 3
24 3
25 3
26 3
27 3
28 3
29 3
30 3
31 2
32 2
33 1
34 2
35 2
36 1
37 1
38 1
39 2
40 2
41 2
42 2
43 2
44 2
45 2
46 1
47 1
48 1
49 1
50 1
51 1
52 1
53 2
54 2
55 2
56 2
57 2
58 2
59 2
60 2
61 2
62 2
63 2
64 2
65 2
66 2
67 2
68 2
69 2
70 2
71 2
72 2
73 2
74 2
75 2
76 2
77 2
78 2
79 2
80 2
81 2
82 2
83 2
84 2
85 2
86 2
87 2
88 2
89 2
90 2
91 2
92 2
93 2
94 2
95 2
96 2
97 2
98 2
99 2
};
\addlegendentry{DRAM}
\end{axis}

\end{tikzpicture}


==> figs/knob1.tex <==
\begin{tikzpicture}[>=latex, every text node part/.style={align=center}]
\node[circle,draw,fill=white, minimum width = 5mm] (a) at (0,0) {};
\filldraw (a.center) circle [radius=.1mm];
\foreach \X in {0,30,...,350}
{\draw (a.\X) -- ++ (180+\X:0.1);}
\draw[-,ultra thick] (a.center) -- (a.90);
\end{tikzpicture}

==> figs/knob2.tex <==
\begin{tikzpicture}[>=latex, every text node part/.style={align=center}]
\node[circle,draw,fill=white, minimum width = 5mm] (a) at (0,0) {};
\filldraw (a.center) circle [radius=.1mm];
\foreach \X in {0,30,...,350}
{\draw (a.\X) -- ++ (180+\X:0.1);}
\draw[-,ultra thick] (a.center) -- (a.130);
\end{tikzpicture}

==> figs/knob3.tex <==
\begin{tikzpicture}[>=latex, every text node part/.style={align=center}]
\node[circle,draw,fill=white, minimum width = 5mm] (a) at (0,0) {};
\filldraw (a.center) circle [radius=.1mm];
\foreach \X in {0,30,...,350}
{\draw (a.\X) -- ++ (180+\X:0.1);}
\draw[-,ultra thick] (a.center) -- (a.300);
\end{tikzpicture}

==> figs/motivation/temp_colormap.tex <==
\begin{tikzpicture}
    \begin{axis}[
        hide axis,
        scale only axis,
        height=0pt,
        width=0pt,
        colorbar,
        colorbar style={
            ytick={0.75,0.8,0.85,0.9,0.95},minor ytick={},ylabel near ticks,ylabel={Normalized energy},
           height = 4cm,
            yticklabel pos=left
        },
        point meta max=0.95,
        point meta min=0.72,
        colormap={mymap}{[1pt]
            rgb(0pt)=(0,0.407843137254902,0.215686274509804);
            rgb(1pt)=(0.101960784313725,0.596078431372549,0.313725490196078);
             rgb(2pt)=(0.4,0.741176470588235,0.388235294117647);
            rgb(3pt)=(0.650980392156863,0.850980392156863,0.415686274509804);
            rgb(4pt)=(0.850980392156863,0.937254901960784,0.545098039215686);
             rgb(5pt)=(1,1,0.749019607843137);
            rgb(6pt)=(0.996078431372549,0.87843137254902,0.545098039215686);
            rgb(7pt)=(0.992156862745098,0.682352941176471,0.380392156862745);
            rgb(8pt)=(0.956862745098039,0.427450980392157,0.262745098039216);
            rgb(9pt)=(0.843137254901961,0.188235294117647,0.152941176470588);
            rgb(10pt)=(0.647058823529412,0,0.149019607843137)
        },
        ]
    \addplot [draw=none] coordinates {(0,0)};
\end{axis}
\end{tikzpicture}
